Cross-TOP: Zero-Shot Cross-Schema Task-Oriented Parsing

Deep learning methods have enabled task-oriented semantic parsing of increasingly complex utterances. However, a single model is still typically trained and deployed for each task separately, requiring labeled training data for each, which makes it challenging to support new tasks, even within a single business vertical (e.g., food-ordering or travel booking). In this paper we describe Cross-TOP (Cross-Schema Task-Oriented Parsing), a zero-shot method for complex semantic parsing in a given vertical. By leveraging the fact that user requests from the same vertical share lexical and semantic similarities, a single cross-schema parser is trained to service an arbitrary number of tasks, seen or unseen, within a vertical. We show that Cross-TOP can achieve high accuracy on a previously unseen task without requiring any additional training data, thereby providing a scalable way to bootstrap semantic parsers for new tasks. As part of this work we release the FoodOrdering dataset, a task-oriented parsing dataset in the food-ordering vertical, with utterances and annotations derived from five schemas, each from a different restaurant menu.

==> abstract.tex <==
\begin{abstract}
In recent years, deep learning methods  have enabled task-oriented semantic parsing of increasingly complex utterances. However, a single model is still typically trained and deployed for each task separately, requiring labeled training data for each, which makes it challenging to support new tasks, even within a single business vertical. In this paper we describe Cross-TOP (Cross-Schema Task-Oriented Parsing), a zero-shot method for complex semantic parsing in a given vertical. With Cross-TOP, a single cross-schema parser is trained and services an arbitrary number of tasks, seen or unseen, within the same business vertical.  We show that Cross-TOP can achieve high-accuracy semantic parsing for a previously unseen task in the vertical of interest, without requiring any training data at all from the new task, thereby providing an effortless way to bootstrap semantic parsers for brand new tasks. As part of this work, we release a new task-oriented parsing dataset in the food-ordering vertical, with utterances and annotations derived from five schemas, each from a unique restaurant menu. 
\end{abstract}


==> conclusion.tex <==
\section{Conclusion}

In this work we evaluated Cross-TOP, a zero-shot approach to cross-schema task-oriented parsing.
Cross-TOP is the first of its kind, a neural task-oriented modeling approach that can parse unseen tasks of different schema.
In addition, the approach produces output that is easily resolved to a representation that can
be executed by a downstream process, such as a voice assistant speechlet, or a kitchen staff in the case of
the food-ordering domain.

Through experimentation on a new task-oriented parsing food-ordering dataset that we release, we show that
indeed Cross-TOP method achieves good zero-shot results.  The only data necessary for parsing a new task is a
schema made up of intents, slots, entities and aliases.  We see that the method relies on a set of aliases to bridge
the gap between entities and user phrasings of the entities, and show how important it is to iterate and update
the schema as users begin querying and making requests in the system.  Updating the schema is a straightforward
process that does not require a model retraining.

An interesting direction could be extending this work by building upon the text-to-SQL focus of
improved encoder-decoder architectures and parsing-specific pretrained language models.  However, we see that the Cross-TOP approach of simply finetuning a readily-available pretrained language model shows promise
and proves to be a useful solution, especially for quickly bootstrapping a parser for a brand new task.



==> dataset.tex <==
\section{Dataset}
Each dataset consist of food order English utterances $U$ for a restaurant
paired with their corresponding semantic parses $Y$.
In addition, each dataset also includes a schema configuration that is based on
the restaurant's menu.
Each schema consists of the following: a set of intents $I$ specifying what kind
of item is being ordered (e.g.\ food or drink), a set of slots $S$ specifying the
attributes of each order such as size and number, a set of entities $E$ which
are items on the menu (sizes small/medium/large, different pizza toppings), and
a set of aliases $A$, which specify how an
entity is called in natural language (English for our dataset).
For example, entity \texttt{regular\_size} may be called \textit{regular} or \textit{regular sized}.
The aliases help bridge the natural language utterances with the execution
environment.

We have five datasets: pizza, burrito, subway, coffee, burger.
The sizes of the datasets are in Table~\ref{tab:data_sizes}.
For each dataset, we hand-crafted the skill configuration $<I, S, E, A>$, with
statistics of each one shown in \ref{tab:schema_stat}

\begin{table}[]
  \begin{tabular}{@{}lllll@{}}
    \toprule
    & \#intents & \#slots & \#entities & \#aliases \\ \midrule
    pizza   &           &         &            &           \\
    burrito &           &         &            &           \\
    subway  &           &         &            &           \\
    coffee  &           &         &            &           \\
    burger  &           &         &            &           \\ \bottomrule
  \end{tabular}
  \caption{Statistics of each schema configuration. }
  \label{tab:schema_stat}
\end{table}


We synthetically generated the training set by XXX \todo{describe the procedure
  for synthesizing the training set utterances and parses}.

For the dev sets, we collected the English utterances on Mechanical Turk by
asking participants to make orders from a given menu based on the defined skill
configuration. The actual instructions for each dataset are in the Appendix.
We discarded utterances that order items that are not on the given menu.
On average, XXX\% of the collected utterances are discarded.
For the remaining utterances, their corresponding semantic parses are manually annotated by the authors.

\begin{table}[]
  \centering
  \begin{tabular}{lrrr}
    \toprule
    Dataset & train & dev & test \\
    \midrule
    Pizza   &       & 348 &      \\
    Burrito &       & 123 &      \\
    Subway  &       & 97  &      \\
    Coffee  &       &     &      \\
    Burger  &       &     &      \\
    \bottomrule
  \end{tabular}
  \caption{Number of examples in each dataset.}
  \label{tab:data_sizes}
\end{table}


Our synthetically generated training set comes in two format, and they differ
in the content of the slot values.
One called TOP-decoupled, which has the aliases in $A$ that are the same as
their mentions in the utterance as the slot values.
The other is EXR, which has the entities in $E$ as slot values.
The TOP-decoupled format can be deterministically converted to EXR by entity resolution.
Our dev set is only annotated with parses in EXR format, since there is no
guarantee that the ways crowdsourced workers mention entities would all be
captured by our list of aliases.


\todo{statistics of the utterances: number of intents/utt, number of
  entities/utt, utterance lengths. maybe in a graph otherwise it's too many
  numbers, 3(train/dev/test) x 5 (5 datasets)}


==> dataset_new.tex <==
\subsection{TOP-FOOD Dataset}

\begin{center}
	\begin{table*}[!hbt]
		{\small
			\centering
			\begin{center}
				\footnotesize
				\hspace*{-0.9cm}
				\begin{tabular}[c]{lcccccl}
					\hline
					Dataset 					& \#Train/Synthetic  &  \#Eval & \#Int & \#Slt & \#SltVals &  Example utterance \\
					\hline
					\textsc{Pizza}                      & 10,000 & 348 & 2 &  11 &  166 & \textit{can i get one large pie with no cheese and a coke} \\
					\textsc{Burrito}                      & 9,982 & 191 & 7 &  12 &  34 & \textit{one carnitas quesadilla with white rice, black beans and a coke} \\
					\textsc{Sub}                       & 10,000 & 162 & 3 &  8 & 62 & \textit{get me a a cold cut combo with mayo and extra pickles} \\
					\textsc{Burger}                      & 0* & 161 & 3 &  9 & 44  &\textit{a vegan burger with lettuce and onions and an order of sweet potato fries} \\
					\textsc{Coffee}                      & 0* & 101 &1 &  10 &  43 &\textit{i would like a regular latte cinnamon iced with one extra espresso shot} \\
					\hline
				\end{tabular}
			\end{center}
			\caption{Food ordering vertical dataset statistics. *\textsc{Burger} and \textsc{Coffee} have no training data as they are used to demonstrate zero-shot learning. \#SltVals is computed by taking the sum of all resolved entities across all different slots for each task.}
			%    Entity resolution was performed on predictions from models trained on TOP and    TOP-Decoupled notations to obtain EXR predictions. PCFG Parser generates EXR directly.}
			\label{table:exrres}
		}
	\end{table*}
\end{center}

\begin{center}
	\begin{table*}[!hbt]
		{\small
			\centering
			\begin{center}
				\footnotesize
				\begin{tabular}[c]{lccc|ccc}

					\hline
													& \multicolumn{3}{c}{Synthetic} & \multicolumn{3}{c}{Human} \\
					\hline
					Dataset 					& \makecell[c]{\#Int per \\ utt}  & \makecell[c]{\#Slot per \\ utt} & \makecell[c]{Avg utt \\ Depth}   &\makecell[c]{\#Int per \\ utt}  & \makecell[c]{\#Slot per \\ utt} & \makecell[c]{Avg utt \\ Depth}  \\ \hline
					\textsc{Pizza}                      & 1.77	&	5.77	&	3.44 & 1.25	&	6.13	&	3.62  \\
					\textsc{Burrito}                      & 1.57	&	6.50	&	3.48 & 1.39	&	5.78	&	3.12 \\
					\textsc{Sub}                       & 1.79	&	6.24	&	3.37 & 1.69	&	5.99	&	3.07\\
					\textsc{Burger}                      & N/A* & N/A* & N/A* & 1.97	&	7.17	&	3.04 \\
					\textsc{Coffee}                      & N/A* & N/A* & N/A* & 1.05	&	5.34	&	3.2 \\
					\hline
				\end{tabular}
			\end{center}
			\caption{Comparing synthetic and human generated data statistics. *\textsc{Burger} and \textsc{Coffee} have no synthetic training data as they are used to demonstrate zero-shot learning.}
			%    Entity resolution was performed on predictions from models trained on TOP and    TOP-Decoupled notations to obtain EXR predictions. PCFG Parser generates EXR directly.}
			\label{table:uttStats}
		}
	\end{table*}
\end{center}

\paragraph{Dataset construction} The TOP-FOOD data subsumes 5 restaurants. For \textsc{sub} and \textsc{burrito} the training portion of the data was syntehtically generated by sampling less than 50 human generated template
for which slots values are then sampled from predefined catalogs.The catalogs and templates will be provided as supplementary material, but a couple example are given in Appendix \ref{appendix:synth}. Those templates and catalogs were randomly sampled up to 10,000 pairs of natural language and target semantic tree, ensuring uniqueness. For \textsc{pizza} we randomly sampled 10,000 utterances ouf ot the 2.5M provided in \cite{pizzaDataset}. The human portion used for evaluation only
was collected throuh Mechanical Turk, where turkers were asked to generate orders from a given menu. See appendix \ref{appendix:mturk} for the detailed instructions. We then annotated the collected utterances to generate the
linearized target semantics. 


\paragraph{Dataset statistics}  Table \ref{table:exrres} presents some summary statistics of the data. All the tasks follow a common structure of intents, slots and slot values, but each task/skill has a different number of intents, slots and catalog sizes. Most notably \textsc{burrito} has 7 distinct indents while \textsc{coffee} is only a single intent task. The choice of design of the task schemata could have been to build a higher level intent for \textsc{burrito} and treat the variety of current intents through an extra slot identifier. Those different design choices accross the same food ordering vertical illustrate that these would also be an arbitray decisions from the restaurant within the same food vertical.

Even if there is variety in design choices across tasks, we can pinpoint some common attributes shared across the schemas of differnt tasks:
\begin{itemize}
 \item[*] target semantics are composed of two types of nodes, namely intents and slots. 
\item[*]  user requests can express an arbitrary number of intents, for example ordering a burrito and drinks, which maps to both \smtt{(BURRITO\_ORDER}) and \smtt{(DRINK\_ORDER}) 
\item[*]  only slots can be children of intent nodes. Intent nodes cannot be children of slot nodes. Any intent can have an arbitrary number of slot children, which can themselves be arbitrarly nested.
\item[*] certain slots are special compositional nodes and could be present to any task: \smtt{(NOT} allows to express negation of a slot, for eg. to remove a topping: \smtt{(NOT (TOPPING mushrooms ))}, while \smtt{(COMPLEX} and \smtt{(QUANTITY} allow to qualify slots like  \smtt{(TOPPING} to express a quantity, for eg \emph{"with a lot of avocado"} would be expressed as \smtt{(COMPLEX (QUANTITY extra )} \smtt{(TOPPING avocado ) ) }.
\end{itemize}

For more details on skills schema please refer to Appendix \ref{appendix:skillSchemas}, while example of actually collected utterances and target semantics are given in Appendix \ref{appendix:dataExamples}. Since the queries are by design multi-intent (mixed orders of dishes, drinks or sides) the depth is incremented by one considering a higher level \smtt{ORDER} parent node that encapsulates the multiple intents. This root note is not displayed in given examples.

\medskip 

Table \ref{table:uttStats} compares relevant statistics on the synthetic and human generated data.



 

==> experiment.tex <==
\section{Experiment}
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{@{}llllllll@{}}
  \toprule
                                                  &                                     & \multicolumn{2}{l}{pizza dev (348 examples)} & \multicolumn{2}{l}{burrito dev (123 examples)} & \multicolumn{2}{l}{subway dev (97 examples)} \\
\multicolumn{2}{l}{constraint decoding?}                                                & no                   & yes                   & no                    & yes                    & no                   & yes                   \\
model                                             & train data                          &                      &                       &                       &                        &                      &                       \\
  \midrule
\multirow{2}{*}{\texttt{BRIDGE}} & pizza                               &                      &                       &                       &                        &                      &                       \\
                                                  & pizza+burrito                       &                      &                       &                       &                        &                      &                       \\
\multirow{4}{*}{Ours}                             & pizza                               &                      &                       &                       &                        &                      &                       \\
                                                  & pizza+burrito                       &                      &                       &                       &                        &                      &                       \\
                                                  & train on pizza, finetune on burrito &                      &                       &                       &                        &                      &                       \\
                                                  & burrito                             &                      &                       &                       &                        &                      & \\
  \bottomrule
\end{tabular}
\end{table}

==> experiment_new.tex <==
\section{Experiment}

\input{dataset_new}

\subsection{Experimental Setup}
To evaluate our model, we train on {\em pizza}, {\em burrito} and {\em sub} tasks and test on {\em coffee} and {\em burger}.
The training(validation) dataset was created by joining all training(dev) data from the three training tasks.
The validation dataset was used for early stopping and model selection.

\paragraph{Implementation Details}
BART \cite{lewis-etal-2020-bart} is the transformer-based pretrained encoder-decoder language model used in our experiments.
BART is pretrained through denoising self-supervised tasks including shuffling, sentence permutation, masking and other corruption techniques.
We use Huggingface BART Large model with 24 encoder/decoder layers and hidden size of 1024,
along with the given hyperparameters and the \texttt{transformers} implementation for finetuning.
Models are trained for 50 epochs with early stopping patience of 4,
using cross-entropy sequence loss using AdamW optimizer with a batch size of 16, learning rate \texttt{1e-05}, linear learning rate scheduler
and warm-up ratio of 0.1.  For generation, beam size was set to 6.  The hyperparameter \texttt{no\_repeat\_ngram\_size}
was set to 0 to disable. We set \texttt{force\_bos\_token\_id=0} to force generation of that token.

Hyperparameter tuning was performed on learning rates [\texttt{5e-04}, \texttt{1e-05}, \texttt{5e-05}, \texttt{1e-06}]
and batch sizes [\texttt{16, 24, 48, 64}] across three seeds.

\paragraph{Vocabulary}
BART uses a byte-pair subword encoding as the tokenizer.  We expand the tokenization vocabulary by adding
input markers \texttt{[I]}, \texttt{[S]} and \texttt{[V]}.  In addition, we adjust the embeddings of the model to
include these three new tokens, with random initialization.

\paragraph{Post-Processing}\label{sec:postprocessing}
Cross-TOP predictions in TOP-Alias format are post-processed into executable representations that match the target format
available in the ground truth test data for each task.  This includes mapping leaf slots from alias to entity tokens using the (alias, entity)-pairs
availabe in the schema data.  In addition, if the slot \texttt{NUMBER} wasn't included in an intent subtree, it was added with the
default slot value of 1.




==> intro.tex <==
\section{Introduction}
%Task-oriented semantic parsing is an important part of virtual assistants, turning a user's request into a meaningful
%representation used by the backend system.

Propelled by deep learning, task-oriented parsing has recently made significant strides, moving away from flat intents and slots towards more complex tree-based semantic structures 
that can represent meaning compositionally \cite{gupta2018semantic,aghajanyan-etal-2020-conversational,rongali2020don}. 
However, most semantic parsing systems remain task-specific: they can only produce representations with the set of intents and slots seen during training.
To support multiple tasks, this approach requires collecting training data, training, and maintaining a model for each task separately. 
This is quite costly when multiple tasks need to be supported, as is usually the case for digital voice assistants such as Alexa and Google Assistant, which may need to support hundreds or thousands of different tasks in a given business vertical (e.g., restaurants in the food-ordering vertical, hotels in the travel vertical, and so on). 

In this paper we present a single semantic parser that supports multiple tasks from a given business vertical. This methodology is an efficient way 
to scale across many different tasks within a vertical. User requests from the same vertical have lexical and semantic similarities; their main differences 
lie in their unique schemas (e.g., different types of menus in the food-ordering vertical). For this reason, we refer to this work as {\em cross-schema task-oriented parsing} (Cross-TOP).
In the food-ordering domain, for example, a customer may request a main dish with various options and possibly a drink and a side. However, 
depending on the restaurant menu, the output semantic representations can differ greatly; see Figure~\ref{fig:intro_example}.

\begin{figure}[h!]
    \centering
%    \includegraphics[width=0.48\textwidth]{figures/zsp_intro_example_2.png}
    \includegraphics[width=0.48\textwidth]{figures/ctop.png}
    \caption{The Cross-TOP parser processes utterances from multiple tasks with different schemas.
    For the food-ordering domain, this example shows pizza and burrito ordering tasks processed by the same parser.}
    \label{fig:intro_example}
\end{figure}

Cross-TOP is a system for zero-shot cross-schema task-oriented parsing. The approach makes use of a powerful pretrained transformer-based encoder-decoder 
language model, with schema-specific context added to the input along with the utterance.  In this way, the model learns to generate parses 
for a new, unseen task, by attending to the schema in the input rather than by needing to see it during training.
We show that this approach is quite effective and provides a quick solution to the practical problem of bootstrapping semantic parsers 
for new tasks within a vertical, using a single model in production.

The parser is trained on a number of initial tasks, where each task has some training data available. Moreover, we assume that every task has a unique {\em schema}. 
That schema consists of all possible intents and slots for the task at hand; both intents and slots can be arbitrarily nested (compositional). 
For every slot $S$, the schema also includes natural-language phrases for the various values of $S$. Cross-TOP uses constrained decoding to ensure that it generates well-formed parses that can be resolved to executable representations by the back end. 

%The only known work for zero-shot cross-schema task-oriented parsing is in solving the slot filling
%sub-problem for non-hierarchical representations~\cite{bapna2017zeroshot, siddique2021linguisticallyenriched, du-etal-2021-qa}.
Most zero-shot cross-schema semantic parsing work has been in the context of the Text-to-SQL problem~\cite{zhong-etal-2020-grounded, lin-etal-2020-bridging, wang-etal-2020-rat, rubin-berant-2021-smbop-semi, DBLP:journals/corr/abs-2009-13845, gan2021natural}.
%(see Section~\ref{sec:related}).
Cross-schema task-oriented parsing introduces its own challenges.
In SQL, the schemas are database schemas, and the parser trained on some initial databases is then evaluated on another database. 
There is a lot of invariant structure among the different schemas and their relationship to utterance phrases. However, in task-oriented parsing 
for the food-ordering domain, the only invariant structures are the parentheses, and some lexical overlap among the intents and slots. 
Therefore, cross-schema parsing in general is much more challenging for task-oriented parsing, although restricting the scope to a given vertical does introduce more common structure that can prove helpful.

To evaluate our methodology, we focus on tasks in the food-ordering domain, where each task contains examples from a
restaurant with the schema generated from its menu.
Our main contributions are as follows:
\begin{itemize}
    \item We present a new technique for zero-shot intra-vertical cross-schema semantic parsing. 
    \item We release a new task-oriented parsing food-ordering dataset to evaluate our method. The dataset includes examples from five restaurants,
    totaling 30,000 synthetically-generated training examples and 963 human-generated test utterances with labels.
    \item We show that our method achieves up to 73\% exact match accuracy on an unseen ordering task, proving the method's viability for effortlessly handling a new task.
\end{itemize}



==> model.tex <==
\section{Model}
We adapted previous approaches for cross-schema Text-to-SQL parsing to
task-oriented parsing.
As a baseline, we followed the \texttt{BRIDGE} model in \citet{lin-etal-2020-bridging} as
closely as possible.
The \texttt{BRIDGE} model is a seq2seq model with pointer-generator decoders.
To achieve cross-schema parsing, the model takes schema elements as input to the
model, and point to them in the decoding stage.

The \texttt{BRIDGE} model as-is produces TOP-like representations, with no
guarantee that the output representation will be executable.
We modified the model to as a step towards producing executable representations.


\subsection{Problem Definition}
Given a natural language $U$, and a schema configuration consisting of the set
of intents $I$, slots $S$, entity aliases $A$, the parser needs to
generate a parse $Y$ in the TOP-decoupled format.

\subsection{Model Input}
To achieve cross-schema parsing, we
need to pass the schema elements as input to the model.
We followed the format in \texttt{BRIDGE} \citep{lin-etal-2020-bridging} to
include schema elements in the input.
The formulation of \texttt{BRIDGE} is based on table/column/column value in a
database, and they correspond to intent/slot/slot value in task-oriented parsing.


For an utterance $U$, we include the Intents, Slots, and slot Values in the input, serialized into the following format:

\texttt{X = [CLS] U [SEP] [I] i$_1$ [S] s$_{1,i_1}$  [V] a$_{1, s_{1, i_1}}$ [V]
  v$_{2, s_{1, i_1}}$ \ldots [SEP]}

where $i_x \in I$ , $s_{y,x} \in S$, $a_{z,y,x} \in A$.
In the input, the markers \texttt{[I]}, \texttt{[S]}, \texttt{[V]} indicate
that the following tokens are Intent/Slot/Value.
These markers are used as
representations of the following schema elements in the decoder.
The decoder produce an intent $i$ by pointing to its preceeding \texttt{[I]} token.


\subsection{Seq2seq with Pointer-Generator Decoding}
As in \citet{lin-etal-2020-bridging}, the input $X$ is encoded by BERT,
followed by a bi-LSTM to obtain hidden representation $h_X \in \mathbb{R}^{|X|
  \times n}$, where $n$ is the hidden dimension.
The utterance segment of $h_X$ is further encoded by another bi-LSTM to obtain
$h_U \in \mathbb{R}^{|U| \times n}$.
In $h_X$, the positions of the schema markers that can be pointed to by the
decoder are selected and yield the hidden representation of the schema $h_S \in \mathbb{R}^{|S| \times n}$ :

\begin{equation}
  h_S  = [h_X^{i} | X^i \in M ]
\end{equation}

where $M$ is the set of tokens that are pointed by the decoder.
For \texttt{BRIDGE}, $M$ is $\{[I], [S]\}$. For our modification, $M$ is $\{[I],
[S], [V]\}$


The decoder for \texttt{BRIDGE} is a LSTM-based pointer-generator decoder
\citep{see-etal-2017-get} with multi-head attention \citep{NIPS2017_3f5ee243}.
At each timestep, the decoder either generate a token from the syntax vocabulary
$V$, or point to one of the tokens in the encoder hidden representation $h_e$.
For \texttt{BRIDGE}, $h_e$ is $[h_U;h_S] \in \mathbb{R}^{(|U|+|S|) \times n}$.
For our modification, $h_e$ is $h_S \in \mathbb{R}^{(|S|) \times n}$.
In the food ordering datasets, the syntax vocabulary consists of only the parantheses.
The pointing-generating-switch probability is computed in the same way as
\texttt{BRIDGE}, and the last attention head is used for the pointing
probability distribution.

\subsection{Fuzzy-matching}
Since the decoder predicts schema elements by pointing to the schema input, it
is crucial that the input contains all the necessary schema elements.
However, simply putting all the schema elements in the input is not feasible,
including the memory constraint of the GPU hardware and the max sequence
length of BERT of 512 tokens.
Therefore, we need to select the schema elements that are relevant for the
utterance to include in the input.
Using fuzzy string match as in \texttt{BRIDGE}, we include an alias $a \in A$ as a slot
value in the input if $a$ is fuzzy-matched with the utterance.
We then include the slot $s$ that is the parent of the slot value, and the possible
intents $i$ that can be the parent of $s$.

==> model_new.tex <==
\section{Model}
Our proposed Cross-TOP method performs cross-schema task-oriented-parsing using
transfer learning capabilities of a pretrained encoder-decoder language model.
We finetune the pretrained language model on training data from multiple tasks, using carefully crafted input and output formats.
In order to enable the model to generalize to a new unseen task,
we format model inputs to include task schema.  We represent the output as
schema-aware linearized tree structures and add constrained decoding so that predictions
can be easily post-processed into executable representations for downstream use.

\subsection{Problem Definition}
Given a natural language $U$, and a schema configuration consisting of the set
of intents $I$, slots $S$, entity aliases $A$, the parser needs to
generate a parse $Y$ in the TOP-Alias format, specified in Section~\ref{sec:output}.

\subsection{Model Input}\label{sec:input}
To achieve zero-shot cross-schema parsing, we
pass the schema elements as input to the model.
We mimic the format in BRIDGE \citep{lin-etal-2020-bridging} to
include schema elements in the input.
The formulation of BRIDGE is based on table/column/column value in a
database, and they correspond to intent/slot/slot value in task-oriented parsing.

For an utterance $U$, we include the intents, slots, and slot values in the input, serialized into the following format:

\medskip

\texttt{U [I] i$_1$ [S] s$_{1,i_1}$  [V] a$_{1, s_{1, i_1}}$
    [V] a$_{2, s_{1, i_1}}$  \ldots [S] s$_{2,i_1}$  [V] a$_{1, s_{2, i_1}}$  \ldots}

\medskip

where $i_x \in I$ , $s_{y,x} \in S$, $a_{z,y,x} \in A$.
Markers \texttt{[I]}, \texttt{[S]}, \texttt{[V]} indicate the tokens following are intents, slots and slot values, respectively.

\subsection{Model Output}\label{sec:output}
The model is trained to generate a parse $Y$ formatted in hierarchical notation TOP-Alias, based on the
TOP notation \cite{gupta-etal-2018-semantic-parsing}.
TOP-Alias format prunes all semantically unnecessary leaves, like {\em decoupled } TOP \cite{aghajanyan-etal-2020-conversational},
only keeping leaf slots.  However, the TOP-Alias leaf slots are alias tokens from $A$
instead of utterance tokens.  Because schema data include many-to-one alias-to-entity pairs, the TOP-Alias format can be
trivially post-processed into an executable representation by substituting entity for alias in the predicted parse $Y$.
An example is given at the end of this section.

Note the model input also includes aliases as slot values (Section~\ref{sec:input}), and as such
the transformer encodes utterance and alias tokens together.
This allows the decoder to attend to the user's request and generate the corresponding alias tokens as leaf slots in the TOP-Alias output,
even for unseen schema.

This separation of utterance, alias and entity formatting is an important modeling choice.  Ultimately the goal of our system
is to execute a user's request, specified in their utterance.  However, if the utterance is parsed in a way that cannot
be mapped to an actual entity in the backend system, the request cannot be executed. Not just any utterance token can be
a valid, executable entity downstream.  This is why utterance tokens aren't formatted as leaf slots in the model output.

Another alternative could have been formatting entities as leaf slots.
However, if entities were part of the input schema instead of aliases,
a more rigid data requirement would be necessary, where entities are named with natural language-based meaningful words so that
utterances can be matched to the entity in the pretrained language model encoding.
Some text-to-SQL cross-schema systems follow this pattern and require "natural language" table or column names to properly
contextualize utterance representations to schema elements~\cite{zhong-etal-2020-grounded}.
However, this requirement is rarely met in practice.
Instead, we use alias data $A$ in our schema to bridge the gap between natural language phrasing of an entity and the
entity name itself.  This is similar to including database cell values as part of the input for lexical schema linking~\cite{lin-etal-2020-bridging}.
Our approach also allows for multiple phrasings (aliases) for a single entity.

See the burrito example in Figure~\ref{fig:intro_example}.  The customer wants to order "guac" on their burrito.  The system's entity
name for this topping may be \texttt{TOPPING1}, while the schema perhaps includes the (alias, entity)-pair \texttt{(guacamole, TOPPING1)}.
A correct output parse is shown, where the leaf slot contains alias \texttt{guacamole}. This predicted parse can then be post-processed to
generate an executable representation where the alias \texttt{guacamole} is replaced by the entity \texttt{TOPPING1}.

\subsection{Constrained Decoding}
One of the advantages of Cross-TOP lies in its ability to generate TOP-Alias by attending to the intermediate structured schema input intents,
slots and aliases. A tries-based entity resolution system will be able to resolve into a fully executable logical form.
Generating TOP-Alias format provides one more advantage in that the decoding can be constrained to only generate valid parses according to a pre-defined grammar.
For example the generated string \texttt{(PIZZA\_ORDER (SIZE mushrooms ) )} is not valid according to the grammar as the alias \texttt{mushrooms} is not a
a valid catalog entry for the slot \texttt{SIZE} as per definintion of the skill schema. Multiple constraints can be implemented along those lines. 

In this work, we implement a parenthesis balancing constraint to ensure well-formed trees, as well as a set of valid next token constraints, where each
subword that can be generated by the decoder has a corresponding entry in a dicitonnary mapping it to the valid next token that can follow from it.
This allows us to restrain the size of the vocab from which a subword can be generated at each decoding step,
based on the decoding history up to current timestep.

These task specific dictionaries are programatically built given the schemata of te task. The construction of this dictionary allows only the following transitions:

\footnotesize{
\[
\left\{
\begin{tabular}{lll}
\texttt{BOS} & $\rightarrow$ & \{$"( X "$,  $X$ = valid intent \} \\
$"("$ & $\rightarrow$ &  \{ $X$,  $X$ = valid intent or slot\} \\
$")"$ & $\rightarrow$ & \{$")"$ or $"("$ or \texttt{EOS} \} \\
intent  & $\rightarrow$   & \{$X$, $X$ = a valid slot  \} \\
slot & $\rightarrow$   & \{$X$,  $X$ = compatible alias \} \\
\texttt{(COMPLEX}   & $\rightarrow$ &\texttt{(QUANTITY}
\end{tabular}
\right.
\]
}

\medskip

\normalsize
At a higher level, these ensure that the generated output will have well-formed trees, starting with intents and then slot and slot value (alias), and forcing the slot-alias combination to be in the catalogs. Additionaly this forces the only slot to be preceded by the \texttt{(COMPLEX} slot to be \texttt{(QUANTITY}. 

\medskip

One could think of imposing more constraints, for example allowing only intent to slot combinations, or allowing only negatable slots after \texttt{(NOT} since some of these, like \texttt{SIZE} cannot be negated. In general constraints to ensurel tree structure abides by a pre-defined grammar could be added, but not all constraints can be easily formulated with dictionary based next valid tokens. We defer these to future work as we did not see these occurring too often by manual inspection.

\medskip

Section~\ref{section:results} gives a quantitative and qualitative idea of the the benefits of constrained decoding in the zero-shot setting.

\subsection{Fuzzy Matching}
Since the decoder learns to predict schema elements it attends to in the model input, it
is crucial that the input contains all the necessary schema elements.
However, simply putting all the schema elements in the input is not feasible,
including the memory constraint of the GPU hardware and the max sequence
length of the pretrained language model input.
Therefore, we need to select the schema elements that are relevant for the
utterance to include in the input.
Using fuzzy string match as in BRIDGE~\cite{lin-etal-2020-bridging}, we include an alias $a \in A$ as a slot
value in the input if $a$ is fuzzy-matched with the utterance.
We then include the slot $s$ that is the parent of the slot value, and the possible
intents $i$ that can be the parent of $s$.

In addition, during input schema generation, we only include the slot \texttt{NUMBER} and corresponding slot values
if the fuzzy-matching algorithm matches aliases for numbers greater than one in the utterance.  This simplifies and cuts down on
additional space in the model input, while not hurting performance.


==> related_work.tex <==
\section{Related Work} \label{sec:related}

\paragraph{Slot Filling}
Traditionally, task-oriented parsing for non-hierarchical intents and slots
has been framed as domain-classification, intent-classification and slot filling component problems~\cite{7846294}.
Within this field works have addressed zero-shot slot filling solutions.
QASF~\cite{du-etal-2021-qa} is a QA-driven solution that extracts slot-filler spans from utterances using a question-answer model.
Both~\citet{bapna2017zeroshot} and~\citet{siddique2021linguisticallyenriched} tag words with slots using slot descriptions
and context-aware representations of the utterance.
These solutions don't solve for hierarchical semantic representations, or multiple intents in a single utterance,
both of which Cross-TOP provides.

\paragraph{Task-Oriented Parsing}
In the more general area of task-oriented parsing where hierarchical representations are featured, the authors are not aware of
other zero-shot cross-schema work. There is work in the few-shot setting~\cite{chen-etal-2020-low}, where data from multiple domains are used during an additional
stage of fine-tuning along with meta-learning to improve on the few-shot task.


\paragraph{Text-to-SQL}
Some of the most relevant related zero-shot work is in the text-to-SQL semantic parsing area.  In this area, a challenging
dataset, SPIDER~\cite{yu-etal-2018-spider}, is the most common dataset to test zero-shot solutions. The most promising of these
solutions frame the problem as a translation problem, translating the utterance to a semantic representation, and solve it
using neural encoder-decoder architectures.

The GAZP~\cite{zhong-etal-2020-grounded} method generates synthetic training data for the new schema environment and
requires a retraining of the neural parser, not making it as convenient of a zero-shot method. RAT-SQL~\cite{wang-etal-2020-rat} moves away from needing to
retrain the parser, and focuses on better encoding of the schema.  It encodes utterance and schema together in such a way
that tokens from a single schema element are represented in a single encoded vector contextualized with the utterance.  It includes explicit relations
between utterances and columns if utterance words occur as column values.
BRIDGE \citep{lin-etal-2020-bridging} also encodes the utterance and schema together, and augments with anchor texts, which
are database values from tables to better bridge utterance tokens to database tables, columns and values.  This is the
main motivation for our work, where we utilize aliases to bridge utterance tokens to intents, slots and entities for a lexical encoding.
SMBOP~\cite{rubin-berant-2021-smbop-semi} focuses on improving the decoder, employing a semi-autoregressive bottom-up tree-based decoder.

These improved neural architectures are boosted with data augmentation and better pretrained language models.
GRAPPA~\cite{DBLP:journals/corr/abs-2009-13845} pretrains a language model from unstructured and structured table data
with objectives for semantic parsing, then fine-tune on final task.
There is also the work of \citet{Shi_Ng_Wang_Zhu_Li_Wang_Nogueira} that pretrains a language model, like GRAPPA,
but uses more innovative semantic parsing objectives based on error analysis from RAT-SQL+BERT on the SPIDER dataset.

Finally in \citet{gan2021natural}, improvements are made with a revised SQL-based intermediate representation that is closer to natural language,
but can be post-processed into SQL for executable representations.  The focus on executable representations is shared with our work.

==> result.tex <==
\section{Results and Analysis}\label{section:results}
Zero-shot results on coffee and burger tasks are shown in Table~\ref{table:main_results}.

\begin{center}
    \begin{table}[!hbt]
    {\small
    \centering
    \begin{center}
        \begin{tabular}[c]{lll}
            \toprule
                                %& \multicolumn{2}{c}{\textbf{TOP-FOOD Task}}   \\
                                & Burger & Coffee \\
            \cmidrule(lr){2-3}
            Cross-TOP (unconstrained)     & 53.00 & 33.33 \\
            Cross-TOP       & 73.33 & 54.79 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Zero-shot Unordered EM accuracy, averaged over 3 seeds}
    \label{table:main_results}
    }
    \end{table}
\end{center}

Unordered Exact match accuracy (EM) is used to measure results.
Unordered EM checks for an exact match between ground truth and
prediction trees, where sibling order doesn't matter.  The results shown compare executable representations,
predictions after post-processing (Section~\ref{sec:postprocessing}).
Cross-Top zero-shot results on {\em coffee} and {\em burger} tasks show EM greater than 50\%. While there is room for improvement, this
result shows Cross-TOP as a viable solution for bootstrapping semantic parsing for a new task.

\paragraph{Constrained decoding helps}
From Table~\ref{table:main_results} we see that constrained decoding boosts performance on the burger and coffee tasks,
from 53\% to 73\% Unordered EM and from 33\% to 55\% respectively. Because the output format is completely schema-aware with known intents, slots and
aliases, it is possible to use this information to guide the decoder generation for improved results.

Manual analysis of 15 utterances each from burger and coffee 
where the generated TOP-Alias predictions from the 
unconstrained and constrained decoding differ showed that 93.3\% (burger) 
and 60\% (coffee) of the utterances had at least one invalid slot and slot value (alias) 
combination in the unconstrained decoding prediction 
that was fixed by constrained decoding. 
While all 15 utterances are incorrectly parsed by the unconstrained decoder, 
constrained decoding generates the correct TOP-Alias prediction in 
60\% and 33.3\% of the cases respectively. We show some examples of how 
constrained decoding helps in Table~\ref{table:constrained_decoding_helps_examples}. 

\begin{table*}[!hbt]
  \centering {\scriptsize   
	\begin{tabular}{|l|l||l|l|}
		\hline
		\textbf{Datset} & \textbf{Natural Language Utterance} & 	\textbf{TOP-Alias prediction using unconstrained decoding} & 	\textbf{TOP-Alias prediction using constrained decoding} \\	\hline
		 \textsc{burger} &\makecell[l]{i'll have a hamburger topped with bacon \\ and ketchup along with a large coke \\ and large order of french fries} & \makecell[l]{\smtt{(MAIN\_DISH\_ORDER} \smtt{(NUMBER a )} \\ \smtt{(MAIN\_DISH\_TYPE hamburger )} \\ \smtt{(TOPPING bacon )} \\ \smtt{(TOPPING ketchup ))} \\ \smtt{(DRINK\_ORDER} \smtt{(NUMBER a )} \\ \smtt{(SIZE large )} \\ \smtt{(DRINK\_TYPE coke ))} \\ \smtt{(SIDE\_ORDER} \smtt{(\textcolor{red}{NUMBER large} )} \\ \smtt{(SIDE\_TYPE french fries ))} } & \makecell[l]{\smtt{(MAIN\_DISH\_ORDER} \smtt{(NUMBER a )} \\ \smtt{(MAIN\_DISH\_TYPE hamburger )} \\ \smtt{(TOPPING bacon )} \\ \smtt{(TOPPING ketchup ))} \\ \smtt{(DRINK\_ORDER} \smtt{(NUMBER a )} \\ \smtt{(SIZE large )} \\ \smtt{(DRINK\_TYPE coke ))} \\ \smtt{(SIDE\_ORDER} \smtt{(\textcolor{green}{NUMBER a} )} \\ \smtt{(\textcolor{green}{SIZE large} )} \\ \smtt{(SIDE\_TYPE french fries ))} } \\ \hline
		 \textsc{coffee} &\makecell[l]{i'd like an iced cappuccino with \\ caramel syrup and whipped cream} & \makecell[l]{\smtt{(DRINK\_ORDER} \smtt{(NUMBER an )} \\ \smtt{(\textcolor{red}{STYLE iced cappuccino} )} \\ \smtt{(TOPPING caramel syrup  )} \\ \smtt{(TOPPING whipped cream ))} } & \makecell[l]{\smtt{(DRINK\_ORDER} \smtt{(NUMBER an )} \\ \smtt{(\textcolor{green}{STYLE iced} )} \\ \smtt{(\textcolor{green}{DRINK\_TYPE cappuccino} )} \\ \smtt{(TOPPING caramel syrup )} \\ \smtt{(TOPPING whipped cream ))} } \\ \hline		
	\end{tabular}
}
	\caption{Example natural language utterances showing how constrained decoding helps fix invalid slot and slot value (alias) combinations.} \label{table:exmap}
    \label{table:constrained_decoding_helps_examples}
\end{table*}

\paragraph{More training tasks are better}
Table~\ref{table:training_tasks} shows results from an ablation study varying the number of training tasks.
The results for training on one task are an average over three models, trained on {\em pizza}, {\em burrito}
and {\em sub} tasks separately.  Likewise, results for training on two tasks are an average of three models, one trained on
{\em pizza+burrito}, one on {\em burrito+sub} and the other on {\em pizza+sub}. It can be observed going from 1 to 2 tasks doubles performance for Burger, and using 3 tasks almost triples the performance for both zero-shot datasets. As more tasks are used
as training data, the better zero-shot results become.  This is intuitive, as the model continues to learn general patterns
and perform better on unseen tasks.

\begin{center}
    \begin{table}[!hbt]
    {\small
    \centering
    \begin{center}
        \begin{tabular}[c]{lll}
            \toprule
            %& \multicolumn{2}{c}{\textbf{TOP-FOOD Task}}   \\
            & Burger & Coffee \\
            \cmidrule(lr){2-3}
            1 Task       & 25.40 & 19.91 \\
            2 Tasks      & 52.38 & 33.99 \\
            3 Tasks      & 73.29 & 54.79 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Average zero-shot Unordered EM accuracy, trained on varying number of training tasks, averaged over 3 seeds.}
    \label{table:training_tasks}
    }
    \end{table}
\end{center}

\paragraph{Task schema in the input is necessary}
In order to determine how much Cross-TOP relies on the task schema 
being present in the input, we ran an ablation study where 
we created train/dev/test sets with no task schema included in the input. 
Table~\ref{table:task_schema_is_necessary} shows the performance of Cross-TOP on such test sets.

\begin{center}
    \begin{table}[!hbt]
    {\small
    \centering
    \begin{center}
        \begin{tabular}[c]{lll}
            \toprule
            %& \multicolumn{2}{c}{\textbf{No Schema Inputs}}   \\
                                        & Burger & Coffee \\
            \cmidrule(lr){2-3}
            Cross-TOP                   & 73.29 & 54.79 \\
            Cross-TOP (No schema in input)   & 26.50 & 31.68 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Unordered EM accuracy results with no schema information included in inputs, averaged over 3 seeds}
    \label{table:task_schema_is_necessary}
    }
    \end{table}
\end{center}

We can see that the accuracy drops by 46\% and 23\% absolute 
for burger and coffee respectively.
A manual analysis of the predictions from Cross-TOP (No schema in input) 
shows that in an overwhelming majority of cases, it only generates 
intents and slots that it has seen before in training 
and thus fails to correctly parse utterances that have an unseen intent/slot. 
To quantify this, we created a test set of 108 utterances that was a subset of 
the original test set for the burger task with at least one intent/slot 
different from the schemas of all the tasks Cross-TOP was trained on. 
The accuracy of Cross-TOP (No schema in input) on this new test set was 4\% EM, 
compared to 64\% EM by Cross-TOP. 
This makes sense because in a zero-shot setting 
where the model is tested on an previously unseen schema, the model has no idea 
of the underlying schema intents/slots it needs to generate 
without being able to refer to the schema.

\paragraph{Missing schema in the input is a challenge}
Cross-TOP also relies on input with complete schema. If in our burrito example from Figure~\ref{fig:intro_example} the
fuzzy-match algorithm didn't locate and include the alias \texttt{guacamole} in the input, then it would become harder for the model to
get the correct prediction tree to include \texttt{(TOPPING guacamole)}.  Sources of incomplete input schema are either
missing aliases or failures in the fuzzy-match algorithm.

One example of missing schema that causes many errors in {\em sub} task, for example, is the lack of alias \texttt{mayo} for the
entity \texttt{regular\_mayonnaise}, and inability for the implemented fuzzy-match algorithm to match the utterance token
"mayo" to the available alias \texttt{mayonnaise}.  While in reality, missing aliases can easily be added to the system to
resolve these types of errors, some level of missing schema input will exist as the schema matures with use.
Table~\ref{table:missing} shows the number of dev/test examples with missing schema input.  For example, int the {\em coffee}
task 7\% of the examples have missing schema in the input, all of which will be nearly impossible to get correct by our model.

\begin{center}
    \begin{table}[!hbt]
    {\small
    \centering
    \begin{center}
        \begin{tabular}[c]{lcc}
            \toprule
            %& \multicolumn{2}{c}{\textbf{Missing Schema Inputs}}   \\
            & Number & Percent \\
            \cmidrule(lr){2-3}
            pizza       & 14 & 4\% \\
            burrito     & 11 & 5\% \\
            sub         & 35 & 23\% \\
            coffee      & 8  & 7\% \\
            burger      & 2 &  1\% \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Number of examples of dev/test input with missing schema}
    \label{table:missing}
    }
    \end{table}
\end{center}

To analyze this type of error we created oracle schema dev/test sets, where all required schema were included in the input.
Results in Table~\ref{table:oracle} show how Cross-TOP performs on these perfect schema inputs.

\begin{center}
    \begin{table}[!hbt]
    {\small
    \centering
    \begin{center}
        \begin{tabular}[c]{lll}
            \toprule
            %& \multicolumn{2}{c}{\textbf{Oracle Schema Inputs}}   \\
                                        & Burger & Coffee \\
            \cmidrule(lr){2-3}
            Cross-TOP                   & 73.29 & 54.79 \\
            Cross-TOP (Oracle Schema)   & 75.57 & 59.41 \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Unordered EM accuracy results with perfect schema information included in inputs, averaged over 3 seeds}
    \label{table:oracle}
    }
    \end{table}
\end{center}

We can observe the accuracy for coffee and burger is slightly improved now that the missing schema elements were added.  In
practice this could mean simply adding aliases to the task schema, so that these new aliases match how users query or
request particular entities. Adding data to the schema doesn't require a model retraining.  The additional schema
elements are used on the fly during inference to form more complete model inputs. These schema-complete inputs are passed
into the same Cross-TOP model, which is then able to generate correct parses.


